Support Recovery for Sparse Deconvolution of Positive Measures

We study sparse spikes deconvolution over the space of Radon measures on $\mathbb{R}$ or $\mathbb{T}$ when the input measure is a finite sum of positive Dirac masses using the BLASSO convex program. We focus on the recovery properties of the support and the amplitudes of the initial measure in the presence of noise as a function of the minimum separation $t$ of the input measure (the minimum distance between two spikes). We show that when ${w}/\lambda$, ${w}/t^{2N-1}$ and $\lambda/t^{2N-1}$ are small enough (where $\lambda$ is the regularization parameter, $w$ the noise and $N$ the number of spikes), which corresponds roughly to a sufficient signal-to-noise ratio and a noise level small enough with respect to the minimum separation, there exists a unique solution to the BLASSO program with exactly the same number of spikes as the original measure. We show that the amplitudes and positions of the spikes of the solution both converge toward those of the input measure when the noise and the regularization parameter drops to zero faster than $t^{2N-1}$.

==> sections/aux/sec-preliminaries-phi-gamma.tex <==
% !TEX root = ../article-asymptotic.tex
\section{Asymptotic of Partial Convolution Matrices}

This section detail asymptotic expansion of various quantities depending on $\Phi_{tx}$ and $\Ga_{tx}$. The proof technics makes use of approximation using Vandermonde and Hermite matrices, in order to use the results of Section~\ref{preliminary}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Injectivity Hypotheses}

\todo{Put part of these definition in the contribution section}

The next definition introduces the only technical hypothesis made on the operator $\Phi$ (except the natural smoothness property imposed to $\phi$) that is useful for our main 
result.

\begin{defn}\label{main-hypothesis}
 For all $k\in\NN^*$, we say that the hypothesis $\Cc_k$ holds if and only if the family $(\phi, \ldots,\phi^{(k-1)})$ is linearly independent in $\Ldeux(\TT)$.
\end{defn}

\begin{lem}\label{gram_invertible}
 If $\Cc_k$ holds, then $F_k^* F_k$ is a symmetric positive \emph{definite} matrix. Moreover this matrix admits a unique square root that we denote $(F_k^*F_k)^{-\frac{1}{2}}$. It is 
 also a symmetric positive definite matrix.
\end{lem}

The hypothesis $\Cc_k$ can be seen as the usual hypothesis made on the frequency cutoff $f_c$ that should be large enough compared to the number of spikes of the input signal when the 
acquisition blur $\Phi$ is modelled by an ideal low-pass filter. Indeed, one has the following proposition

\begin{prop}\label{hyp-fourier}
 If $\Phi$ is the ideal low-pass filter with frequency cutoff $f_c>0$. Then for all $k\in \NN^*$, $\Cc_k$ holds if and only if $k\leq 2 f_c+1$.
\end{prop}
\begin{proof}
 Since $\Phi$ is the ideal low-pass filter with frequency cutoff $f_c$, its kernel $\phi$ is the Dirichlet kernel
 \eq{
	\forall t\in \TT, \ \phi(t)=\sum_{k=-f_c}^{f_c} e^{2i\pi kt}.
 }
 $(\phi, \ldots, \phi^{(k-1)})$ is linearly independent in $\Ldeux(\TT)$ if and only if the family of the Fourier coefficients of $\phi, \ldots, \phi^{(k-1)}$ is linearly independent 
 in $\ell^2(\ZZ)$. But the Fourier coefficients of $\phi^{(i)}$ for $0\leq i\leq k-1$ is an element of $\ell^2(\ZZ)$ supported in $\{j ; \ -f_c\leq j \leq f_c\}$ and given by the 
 following vector of $\RR^{2f_c+1}$
 \eq{
	(2i\pi)^i ((-f_c)^i, (-(f_c-1))^i, \ldots, (-1)^i, 0^i, 1, \ldots, (f_c-1)^i, f_c^i),
 }
 where we use the convention $0^0=1$.
 
 Hence $\Cc_k$ holds if and only if the following matrix has full rank
 \eq{
 \begin{pmatrix}
  1 & -f_c & (-f_c)^2 & \ldots & (-f_c)^{k-1} \\
  1 & -(f_c-1) & (-(f_c-1))^2 & \ldots & (-(f_c-1))^{k-1} \\
  \vdots & \vdots & \vdots & \ddots & \vdots \\
  1 & f_c-1 & (f_c-1)^2 & \ldots & (f_c-1)^{k-1} \\
  1 & f_c & f_c^2 & \ldots & f_c^{k-1}
 \end{pmatrix}
 }
 But this matrix is just $V_k^f$, the Vandermonde matrix of order $k$ of $f$ where 
 \eq{
	f=(-f_c, -(f_c-1), \ldots, -1, 0, 1,\ldots, f_c-1, f_c) \in \RR^{2f_c+1}.
 }
 $V_k^f$ has full rank if and only if $k\leq 2f_c+1$ because the coordinates of $f$ are pairwise distincts (since $f_c>0$), hence the result.
\end{proof}

\begin{rem}
 One can generalize Proposition \ref{hyp-fourier} by saying that $\Cc_k$ holds if and only if 
 \eq{
	c_{-\lfloor \frac{k}{2} \rfloor}(\phi), c_{-\lfloor \frac{k}{2} \rfloor+1}(\phi),\ldots c_0(\phi),\ldots, 
	c_{\lfloor \frac{k}{2} \rfloor-1}(\phi), c_{\lfloor \frac{k}{2} \rfloor}(\phi)
 }
 are nonzeros, where for $i\in \ZZ$, $c_i(\phi)$ is the $i$-th Fourier coefficient of $\phi$.
\end{rem}

Later on we will deal with quantities that involve $(\Phi_{tx}^* \Phi_{tx})^{-1}$ and $(\Ga_{tx}^* \Ga_{tx})^{-1}$ for $t>0$ small. But first, one has to justify the invertibility of 
these matrices. Although it is true that $\Ga_x$ has full column rank (for all $x \in \TT^n$ with pairwise distinct coordinates) in the case of the ideal low-pass 
filter (see \cite{duval-exact2013}), it is not clear with a general $\Phi$. However, in this paper we are only interested in the asymptotic behavior of the recovery, using the 
BLASSO, of the measure $m_{a,tx}$ when $t\rightarrow 0$. And it turns out that the condition $\Cc_{n}$ and $\Cc_{2n}$ implies respectively that $\Phi_{tx}^* \Phi_{tx}$ and 
$\Ga_{tx}^* \Ga_{tx}$ are invertible provided that $t$ is small enough, see Theorem \ref{behavior_gramPhi} and \ref{behavior_gramGamma}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Approximate Factorizations}

Now we detail an approximate factorization of $\Phi_x$ and $\Ga_x$ using Vandermonde and Hermite matrices. It enables us to do some useful computations on several 
quantities that appear in our main result.






\begin{prop}
The following factorization holds:
\begin{align}
  \Gamma_t= \Fdn H_t + \Lambda_t D_t,
\end{align}
where 
 \begin{align*}
  \Fdn&=\begin{pmatrix}
  \varphi(\cdot,0) & \varphi'(\cdot, 0) & \ldots & \varphi^{(2n-1)}(\cdot,0)
\end{pmatrix}\\
\Lambda_t&= \begin{pmatrix}
  \left(\int_0^1 (x_i)^{2n}\varphi^{(2n)}(\cdot, stx_i)\frac{(1-s)^{2n-1}}{(2n-1)!}ds\right)_{1\leq i\leq n} & \left(\int_0^1 (x_i)^{2n-1}\varphi^{(2n)}(\cdot, stx_i)\frac{(1-s)^{2n-2}}{(2n-2)!}ds\right)_{1\leq i\leq n} \end{pmatrix}\\
&\\
H_t&=\begin{pmatrix}
  1  & \ldots & 1 & 0 &\ldots & 0\\
  (tx_1) & \ldots & (tx_n) & 1 & \ldots & 1\\
  \vdots & & \vdots & \vdots & & \vdots\\
  \frac{(tx_1)^{2n-1}}{(2n-1)!} & \ldots &   \frac{(tx_n)^{2n-1}}{(2n-1)!}  &   \frac{(tx_1)^{2n-2}}{(2n-2)!}  & \ldots &   \frac{(tx_n)^{2n-2}}{(2n-2)!}  
\end{pmatrix}\\
D_t&= \begin{pmatrix}
  t^{2n} & & & & &\\
  & \ddots & & & &\\
  & & t^{2n} & & &\\
  & & &t^{2n-1} & &\\
  & & & & \ddots &\\
  & & & & & t^{2n-1}
\end{pmatrix}.
\end{align*}
\label{prop-facto}
\end{prop}
\begin{proof}
This factorization is nothing but the Taylor expansions for $\varphi$ and $\varphi'$:
\begin{align}
  \varphi(\cdot, tx_i)&= \varphi(\cdot,0) +(tx_i)\varphi'(\cdot,0)+\ldots +\frac{(tx_i)^{2n-1}}{(2n-1)!}\varphi^{(2n-1)}(\cdot,0)\nonumber\\
  &\qquad \qquad\qquad \qquad \qquad  +(tx_i)^{2n}\int_0^1\varphi^{(2n)}(\cdot, stx_i)\frac{(1-s)^{2n-1}}{(2n-1)!}ds,\label{eq-taylor1}\\
  \varphi'(\cdot, tx_i)&= \varphi'(\cdot,0) +(tx_i)\varphi''(\cdot,0)+\ldots +\frac{(tx_i)^{2n-2}}{(2n-2)!}\varphi^{(2n-1)}(\cdot,0)\nonumber\\
  &\qquad \qquad\qquad \qquad \qquad  +(tx_i)^{2n-1}\int_0^1\varphi^{(2n)}(\cdot, stx_i)\frac{(1-s)^{2n-2}}{(2n-2)!}ds.\label{eq-taylor2}
\end{align}
\end{proof}

%Now, let us define the following matrices/operators\footnote{Attention j'ai chang\'e des notations.}:
%so that\eqref{eq-taylor1} and~\eqref{eq-taylor2} are equivalent to 
\begin{rem}\label{asympt-Lambda}
  The asymptotics of $\Lambda_t$ is given by:
  \begin{align*}
    \lim_{t\to 0} \Lambda_t = \begin{pmatrix}
      \varphi^{(2n)}(\cdot,0)&\ldots &  \varphi^{(2n)}(\cdot,0)    
    \end{pmatrix}\diag\left(\frac{(x_1)^{2n}}{(2n)!}, \ldots, \frac{(x_n)^{2n}}{(2n)!},\frac{(x_1)^{2n-1}}{(2n-1)!},\ldots \frac{(x_n)^{2n-1}}{(2n-1)!}\right)
  \end{align*}
  \label{rem-lambdat}
\end{rem}

\begin{rem}
  There is an immediate factorization of $H_t$ as
  \begin{align*}
    H_t=\diag(1,t,\ldots t^{2n-1})H_1\diag\left(1,\ldots, 1,\frac{1}{t},\ldots \frac{1}{t}\right).
  \end{align*}
  Hence, we notice that
\begin{align*}
  D_tH_t^{-1}& = \diag(t^{2n},\ldots t^{2n},t^{2n-1}\ldots,t^{2n-1})\diag(1,\ldots 1, t\ldots, t)H_1^{-1}\diag\left(1,\frac{1}{t} \ldots ,\frac{1}{t^{2n-1}}\right)\\
  &= H_1^{-1}\diag(t^{2n},\ldots , t ), \quad \mbox{so that }\\
  \Gamma_t H_t^{-1}&= \Fdn + \Lambda_t H_1^{-1}\diag(t^{2n},\ldots , t ).
\end{align*}
\end{rem}
We deduce :
\begin{cor}
The asymptotic behavior of $\Gamma_t$ as $t\to 0$ is given by
  \begin{align}
    \lim_{t\to 0} \Gamma_tH_t^{-1} &= \Fdn.
  \end{align}
Moreover, for $t\neq 0$ small enough, the matrix $(\Gamma_t^*\Gamma_t)$ is invertible and 
\begin{align}
    \lim_{t\to 0} H_t(\Gamma_t^*\Gamma_t)^{-1}H_t^* &= (\Fdn^*\Fdn)^{-1},\\
    \lim_{t\to 0} \Gamma_t(\Gamma_t^*\Gamma_t)^{-1}H_t^{*} &=  \Fdn (\Fdn^*\Fdn)^{-1}.
  \end{align}
In particular, 
\begin{align*}
  \lim_{t\to 0}  \Gamma_t(\Gamma_t^*\Gamma_t)^{-1}\alpha= \Fdn(\Fdn^*\Fdn)^{-1}\delta_0, \qwhereq  \alpha=\begin{pmatrix}
    1\\\vdots \\1\\0\\\vdots\\0
  \end{pmatrix}\qandq\delta_0= \begin{pmatrix}
    1\\0\\\vdots\\0
  \end{pmatrix}.
\end{align*}
\end{cor}






\todo{Fuse what's above with what's below}








\begin{prop}[Factorization of $\Phi_x$ at the order $k$]\label{expan_Phi}
 One has for all $k\in \NN^*$,
 \eq{
	\Phi_x = F_k (V_{k}^x)^* + \epsilon(x),
}
where $F_k = (\phi, -\phi', \frac{1}{2} \phi'', \ldots, \frac{(-1)^{k-1}}{(k-1)!} \phi^{(k-1)})$ stores the successive derivatives of $\phi$ as columns, \textit{i.e.} 
$F_k$ is the matrix of the operator
\eq{
 (a_j)_{j=1}^{k} \mapsto \sum_{j=1}^{k} a_{j} \frac{(-1)^{j-1}}{(j-1)!} \phi^{(j-1)} \in \Ldeux(\TT),
}
and $|\epsilon(x)|_\infty \leq C |x|_\infty^k$ where $C=\frac{\|\phi^{(k)}\|_\infty}{k!}$.
\end{prop}
\begin{proof}
 To do this, we write the following Taylor expansion at the order $k$, for $1\leq i\leq n$ and $t\in \TT$,
\begin{align*}
  \phi(t-x_i)=\sum_{j=1}^{k} \frac{(-x_i)^{j-1}}{(j-1)!} \phi^{(j-1)}(t)  + \frac{(-x_i)^k}{k!} \phi^{(k)}(c_i(t))
  \label{eq-phix-dl}
\end{align*}
for some $c_i(t)\in (t-x_i,t)$ (or $(t,t-x_i)$). Hence the result and $|\epsilon(x)|_\infty \leq \frac{\|\phi^{(k)}\|_\infty}{k!} |x|_\infty^k$.
\end{proof}

\begin{rem}
 If $x\in \TT^n$ is fixed, and if we consider $t x$ for some $t>0$, we get
\eq{
	\epsilon(t x) = O(t^{k}),
}
where $O$ is bounded by a constant which depends on $k$, $|x|_\infty$, and $\|\phi^{(k)}\|_{\infty}$.
\end{rem}

\begin{prop}[Factorization of $\Ga_x$ at the order $k$]\label{expan_Gamma}
 One has for all $k\in \NN^*$,
 \eq{
	\Ga_x = F_{k} (H_{k}^x)^* + \epsilon(x) \qwhereq \epsilon(x)=(\epsilon_1(x) \ \epsilon_2(x)),
}
with $|\epsilon_1(x)|_\infty \leq C_1 |x|_\infty^{k}$, $C_1=\frac{\|\phi^{(k)}\|_\infty}{k!}$ and 
$|\epsilon_2(x)|_\infty \leq C_2 |x|_\infty^{k-1}$, $C_2=\frac{\|\phi^{(k)}\|_\infty}{(k-1)!}$.
\end{prop}
\begin{proof}
 As in Proposition \ref{expan_Phi}, we have $\Phi_x=F_{k} (V_{k}^x)^* + \epsilon_1(x)$ with $|\epsilon_1(x)|_\infty \leq \frac{\|\phi^{k}\|_\infty}{k!} |x|_\infty^{k}$. 
 The Taylor expansion of $\phi'(t-x_i)$ at the order $k$, for $1\leq i\leq n$ and $t\in \TT$ is,
 \eq{
	  \phi'(t-x_i)=\sum_{j=1}^{k-1} \frac{(-x_i)^{j-1}}{(j-1)!} \phi^{(j)}(t)  + \frac{x_i^{k-1}}{(k-1)!} \phi^{(k)}(c_i(t)).
 }
 So $\Phi_x'=F_{k} ((V_{k}^x)')^* + \epsilon_2(x)$ with $|\epsilon_2(x)|_\infty \leq \frac{\|\phi^{k}\|_\infty}{(k-1)!} |x|^{k-1}_\infty$.
 Hence 
 \begin{align*}
  \Ga_x &= \pa{ F_{k} (V_{k}^x)^* \quad F_{k} ((V_{k}^x)')^* } + (\epsilon_1(x) \ \epsilon_2(x) ) \\
	&= F_{k} \pa{ (V_{k}^x)^* \ ((V_{k}^x)')^* } + \epsilon(x) \\
	&= F_{k} (H_{k}^x)^* + \epsilon(x).
 \end{align*} 
\end{proof}

\begin{rem}
 If $x\in \TT^n$ is fixed, and if we consider $t x$ for some $t>0$, we get
\eq{
	\epsilon_1(t x) = O(t^{k}) \qandq \epsilon_2(t x) = O(t^{k-1})
}
where $O$ is bounded by a constant which depends on $k$, $|x|_\infty$, and $\|\phi^{(k)}\|_{\infty}$.
\end{rem}

\begin{rem}
 It is natural to consider the case $k=n$ when we compute quantities depending on $\Phi_x$ and $k=2n$ when we compute quantities depending on $\Ga_x$ because respectively 
 $V_{n}^x$ and $H_{2n}^x$ are invertible. That is what we will do most of the time later on.
\end{rem}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Asymptotics of $(\Ga_{tx}^* \Ga_{tx})^{-1}$}

\begin{defn}
 Let us denote
 \eq{
	\Om_{x}=F_{2n} (H_{2n}^{x})^*.
 }
\end{defn}


 \begin{prop}\label{behavior_gramOm}
  If $\Cc_{2n}$ holds, then 
  \begin{align*}
	(\Om_{tx}^*\Om_{tx})^{-1}&=(H_{2n}^{tx})^{*,-1} (F_{2n}^* F_{2n})^{-1} (H_{2n}^{tx})^{-1}=O\pa{ \frac{1}{t^{4n-2}} } \\
	                         &= \frac{1}{t^{4n-2}} \Hh_x^* (F_{2n}^* F_{2n})^{-1} \Hh_x + O\pa{ \frac{1}{t^{4n-3}} }.
  \end{align*}
 \end{prop}

 \begin{proof}
  From Lemma \ref{gram_invertible}, we know that $F_{2n}^*F_{2n}$ is invertible, so as $H_{2n}^{tx}$, hence $\Om_{tx}^*\Om_{tx}$ is invertible for all $t>0$. We know from 
  Proposition \ref{asympt_vanher} that $(H_{2n}^{tx})^{-1}=\Hh_x/t^{2n-1}+O(1/t^{2n-2})$, hence the results.
 \end{proof}


\begin{thm}\label{behavior_gramGamma}
 If $\Cc_{2n}$ holds, then for $t>0$ small enough $\Ga_{tx}^* \Ga_{tx}$ is invertible and
 \eq{
	(\Ga_{tx}^* \Ga_{tx})^{-1} = \frac{1}{t^{4n-2}} \Hh_x^* (F_{2n}^*F_{2n})^{-1} \Hh_x + O\pa{\frac{1}{t^{4n-3}}}.
 }
\end{thm}
\begin{proof}
 From Proposition \ref{expan_Gamma}, we have the factorization of $\Ga_{tx}$ at order $2n$,
 \eq{
	\Ga_{tx}=\Om_{tx} + \epsilon(tx).
 }
 where $\epsilon(tx)=(\epsilon_1(tx) \ \epsilon_2(tx))$ with $\epsilon_1(tx)=O(t^{2n})$ and $\epsilon_2(tx)=O(t^{2n-1})$.
 
 So
 \eq{
	 \Ga_{tx}^* \Ga_{tx} = \Om_{tx}^*\Om_{tx} + T_{tx},
 }
 where $T_{tx}=\Om_{tx}^* \epsilon(tx) + \epsilon(tx)^* \Om_{tx} + \epsilon(tx)^*\epsilon(tx)$.
 
 Since $\Cc_{2n}$ holds, one has,
 \eq{
	(\Om_{tx}^*\Om_{tx})^{-1}=N_{tx}^*N_{tx} \qwithq N_{tx}=(F_{2n}^*F_{2n})^{-\frac{1}{2}} (H_{2n}^{tx})^{-1} = O\pa{ \frac{1}{t^{2n-1}} }.
 }
 
 Thus,
 \eq{
	\Ga_{tx}^* \Ga_{tx} = N_{tx}^{-1} (I + N_{tx} T_{tx} N_{tx}^*) (N_{tx}^*)^{-1}
 }
 and
 \eq{
	N_{tx} T_{tx} N_{tx}^* = O(t).
 }
 Indeed $N_{tx} \Om_{tx}^* = (F_{2n}^*F_{2n})^{-\frac{1}{2}} F_{2n}^* = O(1)$. Moreover from Proposition \ref{asympt_vanher}, we know that $(H_{2n}^{tx})^{-1}=(A_{tx} \ B_{tx})$ 
 with $A_{tx}=O(1/t^{2n-1})$ and $B_{tx}=O(1/t^{2n-2})$. So $\epsilon(tx)N(tx)^*=(\epsilon_1(tx)A_{tx}^* + \epsilon_2(tx)B_{tx}^*) (F_{2n}^*F_{2n})^{-\frac{1}{2}}=O(t)$.
 Hence
 \begin{align*}
        N_{tx} \Om_{tx}^* \epsilon(tx) N_{tx}^* &= O(t), \\
        N_{tx} \epsilon(tx)^* \Om_{tx} N_{tx}^* &= O(t), \\
        N_{tx} \epsilon(tx)^* \epsilon(tx) N_{tx}^* &= O(t^2).
 \end{align*}

 So for $t>0$ small enough, $\Ga_{tx}^* \Ga_{tx}$ is invertible and
 \begin{align*}
  (\Ga_{tx}^* \Ga_{tx})^{-1} &= N_{tx}^* (I + N_{tx} T_{tx} N_{tx}^*)^{-1} N_{tx} \\
                             &= (\Om_{tx}^*\Om_{tx})^{-1} + \sum_{k=1}^{+\infty} (-1)^k N_{tx}^* \pa{ U_{tx} }^k N_{tx}, \\
                             &= (\Om_{tx}^*\Om_{tx})^{-1} + O\pa{ \frac{1}{t^{4n-3}} }
 \end{align*}
 where $U_{tx} = N_{tx} T_{tx} N_{tx}^*$.
 
 Finally, thanks to Proposition \ref{behavior_gramOm}, one has the expected result.
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Asymptotics $\Ga_{tx}^+$}

\begin{prop}\label{behavior_pinvOm}
 If $\Cc_{2n}$ holds, for $t>0$ small enough,
 \begin{align*}
  \Om_{tx}^+ &= (H_{2n}^{tx})^{*,-1} F_{2n}^+ = O\pa{ \frac{1}{t^{2n-1}} } \\
             &= \frac{1}{t^{2n-1}} \Hh_x F_{2n}^+ + O\pa{ \frac{1}{t^{2n-2}} }.
 \end{align*}
\end{prop}
\begin{proof}
 It is a direct consequence of Proposition \ref{behavior_gramOm} and Proposition \ref{asympt_vanher}.
\end{proof}

\begin{thm}\label{behavior_pinvGa}
 If $\Cc_{2n}$ holds, for $t>0$ small enough,
 \eq{
	\Ga_{tx}^+ = \frac{1}{t^{2n-1}} \Hh_x F_{2n}^+ + O\pa{ \frac{1}{t^{2n-2}} }
 }
\end{thm}
\begin{proof}
 From the proof of the Theorem \ref{behavior_gramGamma}, for $t>0$ small enough,
 \eq{
	(\Ga_{tx}^* \Ga_{tx})^{-1} = (\Om_{tx}^*\Om_{tx})^{-1} + \sum_{k=1}^{+\infty} (-1)^k N_{tx}^* \pa{ T_{tx} }^k N_{tx},
 }
 with $N_{tx}=(F_{2n}^* F_{2n})^{-\frac{1}{2}} (H_{2n}^{tx})^{-1}=O(1/t^{2n-1})$ and $T_{tx}=O(t)$.
 Hence
 \begin{align*}
  \Ga_{tx}^+ &= \Om_{tx}^+ + \sum_{k=1}^{+\infty} N_{tx}^* \pa{ -T_{tx} }^k N_{tx} \Om_{tx}^*  + 
              \sum_{k=1}^{+\infty} N_{tx}^* \pa{ -T_{tx} }^k N_{tx} \epsilon(tx)^*\\
              &= \Om_{tx}^+ + \sum_{k=1}^{+\infty} N_{tx}^* \pa{ -T_{tx} }^k (F_{2n}^*F_{2n})^{-\frac{1}{2}} F_{2n}^* + 
              \sum_{k=1}^{+\infty} N_{tx}^* \pa{ -T_{tx} }^k N_{tx} \epsilon(tx)^*.
 \end{align*}
 As
 \begin{align*}
  \sum_{k=1}^{+\infty} N_{tx}^* \pa{ -T_{tx} }^k (F_{2n}^*F_{2n})^{-\frac{1}{2}} F_{2n}^* &= O\pa{ \frac{1}{t^{2n-2}} }, \\
  \sum_{k=1}^{+\infty} N_{tx}^* \pa{ -T_{tx} }^k N_{tx} \epsilon(tx)^* &= O\pa{ \frac{1}{t^{2n-3}} },
 \end{align*}
 because we know from the proof of Theorem \ref{behavior_gramGamma} that $M_{tx} \epsilon(tx)^*=O(t)$, therefore
 \eq{
	\Ga_{tx}^+ = \Om_{tx}^+ + O\pa{ \frac{1}{t^{2n-2}} }.
 }
 Finally, thanks to Proposition \ref{behavior_pinvOm}, one has the expected result.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Asymptotics of $(\Ga_{tx}^*\Ga_{tx})^{-1}\al_n$}

The study of $(\Ga_{tx}^*\Ga_{tx})^{-1}\al_n$ is important because it represents in some sense a bias associated to the BLASSO estimation procedure.

\begin{thm}\label{behavior_biais}
 If $\Cc_{2n}$ holds, then for $t>0$ small enough,
 \eq{
	(\Ga_{tx}^*\Ga_{tx})^{-1}\al_n = O\pa{ \frac{1}{t^{2n-2}} }.
 }
\end{thm}
\begin{proof}
 From the proof of the Theorem \ref{behavior_gramGamma}, one has for $t>0$ small enough,
 \eq{
	(\Ga_{tx}^* \Ga_{tx})^{-1} \al_n = (\Om_{tx}^*\Om_{tx})^{-1} \al_n + \sum_{k=1}^{+\infty} (-1)^k N_{tx}^* \pa{ T_{tx} }^k N_{tx} \al_n.
 }
 We have
 \eq{
	(\Om_{tx}^*\Om_{tx})^{-1} \al_n = (H_{2n}^{tx})^{*,-1} (F_{2n}^* F_{2n})^{-1} (H_{2n}^{tx})^{-1} \al_n,
 }
 and
 \eq{
	N_{tx}\al_n = (F_{2n}^*F_{2n})^{-\frac{1}{2}} (H_{2n}^{tx})^{-1} \al_n.
 } 
 By definition of the matrix $H_{2n}^{tx}$, $a=(H_{2n}^{tx})^{-1} \al_n$ is a vector so that $P_a(X)$ is the unique polynomial of degree lower than or equal to $2n-1$ such that for 
 all $0\leq i \leq n-1$, $P_a(x_i)=1$ and $P_a'(x_i)=0$. But the constant polynomial equal to $1$ verifies theses properties, hence $P_a=1$ and $a=e_1^{2n}$. 
 Hence, one has $(\Om_{tx}^* \Om_{tx})^{-1}\al_n = (H_{2n}^{tx})^{*,-1} (F_{2n}^* F_{2n})^{-1} e_1^{2n}$ and $N_{tx}\al_n=(F_{2n}^*F_{2n})^{-\frac{1}{2}}$. Hence 
 \eq{
	N_{tx}\al_n = O(1),
 }
 and then
 \eq{
	\sum_{k=1}^{+\infty} (-1)^k N_{tx}^* \pa{ T_{tx} }^k N_{tx} \al_n = O\pa{ \frac{1}{t^{2n-2}} }.
 }
 
 From Lemma \ref{damier_gramFk} and corollary \ref{checkerboard_inverse}, one gets that $(F_{2n}^* F_{2n})^{-1}$ is a checkerboard matrix. Thus the coefficient $(2n,1)$ of 
 $(F_{2n}^* F_{2n})^{-1}$ is equal to zero, therefore the coefficient $2n$ of the vector $(F_{2n}^* F_{2n})^{-1} e_1^{2n}$ is also equal to zero. Hence 
 $\Hh_x (F_{2n}^* F_{2n})^{-1} e_1^{2n} = 0$, which leads to
 \eq{
	(\Om_{tx}^*\Om_{tx})^{-1} \al_n = O\pa{ \frac{1}{t^{2n-2}} }.
 }
 Hence the expected result.
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Asymptotics of $(\Phi_{tx}^*)'' \Ga_{tx}^{+,*} \al_n$}

We aim at computing the vector 
\eq{
	\eta_{V,t}''(tx) = (\Phi_{tx}'')^* \Gamma_{tx}^{+,*} \al_n.
}


\begin{prop}
  Assume that $\Cc_{2n-1}$ holds. Then for all $1\leq i\leq n$
  \begin{align}
    \eta_{V,t}''(tx_i)=\eta_{W}^{(2n)}(0)\left(\prod_{j\neq i} (x_i-x_j)^2\right)t^{2n-2} + o(t^{2n-2}).\label{eq-derivee2n}
  \end{align}
\end{prop}


\begin{proof}
From the Taylor expansion
\begin{align*}
  \varphi''(\cdot,tx_i) &= \varphi''(\cdot,0) + (tx_i)\varphi^{(3)}(\cdot, 0)+\ldots +\frac{(tx_i)^{2n-2}}{(2n)!}\varphi^{(2n)}(0)\\
  & \qquad \qquad \qquad + t^{2n-1}\int_0^{1} (x_i)^{2n-1}\varphi^{(2n+1)}(\cdot,stx_i)\frac{(1-s)^{2n-2}}{(2n-2)!}ds,
\end{align*}
we deduce that 
$\Phi_t''= \tFdn V_t + t^{2n-1}\tilde{\Lambda}_t$, where 
  \begin{align*}
    \tFdn&= \begin{pmatrix}
      \varphi''(\cdot,0) & \ldots \varphi^{(2n)}(\cdot,0)
    \end{pmatrix}, \qquad \tilde{\Lambda}_t=\begin{pmatrix}
      \int_0^{1} (x_i)^{2n-1}\varphi^{(2n+1)}(\cdot,stx_i)\frac{(1-s)^{2n-2}}{(2n-2)!}ds
    \end{pmatrix}_{1\leq i\leq n}\\
    \mbox{and } V_t&= \begin{pmatrix}
      1 & 1 &\ldots & 1\\
      (tx_1) & (tx_2) & \ldots & (tx_n)\\
      \vdots & \vdots & & \vdots \\
      \frac{(tx_1)^{2n-2}}{(2n-2)!} &\frac{(tx_2)^{2n-2}}{(2n-2)!} & \ldots & \frac{(tx_n)^{2n-2}}{(2n-2)!}
    \end{pmatrix}.
  \end{align*}
  Hence, the left hand side of~\eqref{eq-derivee2n} is the $i$-th coordinate of ${\Phi_t''}^*p_{V,t}=V_t^*\tFdn^*p_{V,t} + t^{2n-1}\tilde{\Lambda}_t^*p_{V,t}$. 
  Similarly to Remark~\ref{rem-lambdat}, we observe that 
  \begin{align*}
\tilde{\Lambda_t} = \begin{pmatrix}
      \varphi^{(2n+1)}(\cdot,0)&\ldots &  \varphi^{(2n+1)}(\cdot,0)    
    \end{pmatrix}\diag\left(\frac{(x_1)^{2n-1}}{(2n-1)!}, \ldots, \frac{(x_n)^{2n-1}}{(2n-1)!}\right)+o(1)=O(1).
  \end{align*}

  Since $p_{V,t}=O(1)$ by Corollary~\ref{cor-cvetav}, the term $t^{2n-1}\tilde{\Lambda}_t^*p_{V,t}=o(t^{2n-2})$ is negligible.
It is thus sufficient to study ${\tFdn}^*p_{V,t}$. From the structure of $V_t^*$, let us observe that any term of the form 
 \begin{align}V_t^*\begin{pmatrix}
    o(t^{2n-2})\\  \vdots \\o(t)\\o(1)
  \end{pmatrix}=\begin{pmatrix}
    o(t^{2n-2})\\  \vdots \\o(t^{2n-2})
  \end{pmatrix}\label{eq-proof-second-neglig}\end{align} is also neglible.

\paragraph{Step 1.}
Now, since $\alpha=H_t^{-1}\delta_0$,
\begin{align*}
  p_{V,t}&=\Gamma_t(\Gamma_t^*\Gamma_t)^{-1}\alpha\\
  &=(\Fdn + \Lambda_t  H_1^{-1} \diag(t^{2n},\ldots , t ))(\Fdn^*\Fdn +r_t)^{-1}\delta_0\\
\qwhereq r_t&=\Fdn^*\Lambda_t  H_1^{-1}\diag(t^{2n},\ldots , t )+ \diag(t^{2n},\ldots , t )H_1^{-1,*}\Lambda_t^*\Fdn\\
&\qquad \qquad \qquad +  \diag(t^{2n},\ldots , t )H_1^{-1,*}\Lambda_t^*\Lambda_t  H_1^{-1}\diag(t^{2n},\ldots , t ).
\end{align*}

Let $y_t=(\Fdn^*\Fdn +r_t)^{-1}\delta_0$ (observe that $\lim_{t\to 0}y_t=(\Fdn^*\Fdn)^{-1}\delta_0$, so that $y_t=O(1)$). Then $y_t=(\Fdn^*\Fdn)^{-1}(\delta_0-r_ty_t)$, and 
\begin{align*}
  p_{V,t}&=(\Fdn + \Lambda_t  H_1^{-1} \diag(t^{2n},\ldots , t ))y_t\\
  &= \Fdn(\Fdn^*\Fdn)^{-1}\delta_0 -\Fdn(\Fdn^*\Fdn)^{-1}r_ty_t +\Lambda_t  H_1^{-1} \diag(t^{2n},\ldots , t )y_t.\\
  &= p_W -\Fdn(\Fdn^*\Fdn)^{-1}r_ty_t +\Lambda_t  H_1^{-1} \diag(t^{2n},\ldots , t )y_t,\\
  &= A + B +C,
\end{align*}
where we have replaced $r_t$ with its expression, yielding
\begin{align*}
  A&\eqdef p_W -\Fdn(\Fdn^*\Fdn)^{-1}\diag(t^{2n},\ldots , t )H_1^{-1,*}\Lambda_t^*\Fdn y_t,\\
  B&\eqdef  -\Fdn(\Fdn^*\Fdn)^{-1}\Fdn^*\Lambda_t  H_1^{-1}\diag(t^{2n},\ldots , t )y_t + \Lambda_t  H_1^{-1} \diag(t^{2n},\ldots , t )y_t,\\
  C&\eqdef  -\Fdn(\Fdn^*\Fdn)^{-1}\diag(t^{2n},\ldots , t )H_1^{-1,*}\Lambda_t^*\Lambda_t  H_1^{-1}\diag(t^{2n},\ldots , t ).
\end{align*}

\paragraph{Step 2.} Let us focus on $C$.

We notice that the $n-2$ first lines of the matrix $\tFdn^* \Fdn(\Fdn^*\Fdn)^{-1}$ are the last $n-2$ lines of the matrix $\Fdn^*\Fdn(\Fdn^*\Fdn)^{-1}=I_{2n}$.
The last line depends on the correlations between $\varphi^{(2n)}(\cdot,0)$ and $\varphi^{(j)}(\cdot,0)$ for $0\leq j\leq 2n-1$. As a result:
\begin{align}\label{eq-compagnon}
  \tFdn^* \Fdn(\Fdn^*\Fdn)^{-1}\diag(t^{2n},\ldots , t )&= \begin{pmatrix}
    0 & 0 & t^{2n-2} &0 \\
\vdots&\vdots& 0 &t^{2n-1} & \\
\vdots& \vdots & & \ddots & \ddots& \\ 
0 & 0 & \ldots & \ldots& 0 & t\\
O(t^{2n}) & O(t^{2n-1}) & \ldots & \ldots & \ldots &O(t)
  \end{pmatrix}.
\end{align}
But $H_1^{-1,*}\Lambda_t^*\Lambda_t  H_1^{-1}\diag(t^{2n},\ldots , t )=O(t)$. As a result, $V_t^*\tFdn^* C$ is of the form~\eqref{eq-proof-second-neglig} and is therefore negligible.

\paragraph{Step 3.} Now, we handle the term $B$. 

Notice that $B$ is the orthogonal projection of $\Lambda_t  H_1^{-1} \diag(t^{2n},\ldots , t )y_t$ onto the orthogonal complement of $\Im \Fdn=\Span(\varphi(\cdot,0), \ldots \varphi^{(2n-1)}(\cdot,0))$. Hence, the $n-2$ lines of $\tFdn^*B$ are $0$, whereas the last line is $O(t)$ since $B=O(t)$. As a consequence, $V_t^*\tFdn^*B$ is negligible too. 


\paragraph{Step 4.} It remains to study $A$.

From Remark~\ref{asympt-Lambda} and the fact that $\lim_{t\to 0}y_t=(\Fdn^*\Fdn)^{-1}\delta_0$, one has
\eq{
	\La_t^* F_{2n-1} y_t \underset{t\rightarrow 0}{\longrightarrow} 
		\diag \pa{ \frac{x_1^{2n}}{(2n)!},\ldots,\frac{x_n^{2n}}{(2n)!},\frac{x_1^{2n-1}}{(2n-1)!},\ldots,\frac{x_n^{2n-1}}{(2n-1)!} }
		\begin{pmatrix}
			\dotp{\varphi^{(2n)}}{p_W} \\
			\vdots \\
			\dotp{\varphi^{(2n)}}{p_W}
		\end{pmatrix}.
}
Thus, one gets
\eq{
	H_1^{-1,*} \La_t^* F_{2n-1} y_t \underset{t\rightarrow 0}{\longrightarrow} 
		\eta_W^{(2n)}(0) a \qwhereq a=H_1^{-1,*} 
			\begin{pmatrix}
				\frac{x_1^{2n}}{(2n)!} \\
				\vdots \\
				\frac{x_n^{2n}}{(2n)!} \\
				\frac{x_1^{2n-1}}{(2n-1)!} \\
				\vdots \\
				\frac{x_n^{2n-1}}{(2n-1)!} 
			\end{pmatrix}.
}
$a$ is the vector such that the polynomial $P_a=\sum_{i=0}^{2n-1} \frac{a_{i+1}}{i!} X^i$ is the only one of degree lower or equal than $2n-1$, which verifies $P_a(x_i)=\frac{x_i^{2n}}{(2n)!}$ and $P_a'(x_i)=\frac{x_i^{2n-1}}{(2n-1)!}$ for all $1\leq i \leq n$. We notice that the polynomial 
$\frac{1}{(2n)!}X^{2n} - \frac{1}{(2n)!} \prod_{i=1}^{n} (X-x_i)^2$ meets all the previous conditions, therefore 
\eq{
	P_a=\frac{1}{(2n)!}X^{2n} - \frac{1}{(2n)!} \prod_{i=1}^{n} (X-x_i)^2.
}

From Equation \eqref{eq-compagnon}, we deduce that 
\eq{
	\tFdn^* \Fdn(\Fdn^*\Fdn)^{-1}\diag(t^{2n},\ldots , t ) H_1^{-1,*} \La_t^* F_{2n-1} y_t = 
		\eta_W^{(2n)}(0) \begin{pmatrix}
						a_3 t^{2n-2} + o(t^{2n-2}) \\
						a_4 t^{2n-3} + o(t^{2n-3}) \\
						\vdots \\
						a_{2n} t +o(t) \\
						O(t)
					  \end{pmatrix}.				
}
One thus has
\begin{align*}
	V_t^* \tFdn A &=V_t^* ( \tFdn p_W - \eta_W^{(2n)}(0)  \begin{pmatrix}
													a_3 t^{2n-2} + o(t^{2n-2})\\
													a_4 t^{2n-3} + o(t^{2n-3})\\
													\vdots \\
													a_{2n} t + o(t)\\
													O(t)
					  							\end{pmatrix})
			    =\eta_W^{(2n)}(0) V_t^* \begin{pmatrix}
			    						-a_3 t^{2n-2} + o(t^{2n-2}) \\
									-a_4 t^{2n-3} + o(t^{2n-3})\\
									\vdots \\
									-a_{2n} t + o(t)\\
									1+O(t)
								   \end{pmatrix}
\end{align*}
because $\tFdn p_W=(0 \ \cdots \ 0 \ \eta_W^{(2n)}(0))^*$. So the $i$-th lign of $V_t^* \tFdn A$ is
\eq{
	\pa{ \underbrace{-a_3 - a_4 x_i - a_5 \frac{x_i^2}{2!} - \ldots - a_{2n} \frac{x_i^{2n-3}}{(2n-3)!}}_{-P_a''(x_i)} + \frac{x_i^{2n-2}}{(2n-2)!} } t^{2n-2} + o(t^{2n-2}).
} 
Since $P_a''(x_i)=\frac{x_i^{2n-2}}{(2n-2)!} - \prod_{j\neq i} (x_i-x_j)^2$, by putting all the pieces together, one finally gets the expected result.



\end{proof}








==> sections/aux/sec-preliminaries-vandermonde.tex <==
% !TEX root = ../article-asymptotic.tex
\section{Asymptotic of Vandermonde and Hermite Matrices}
\label{preliminary}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The Vandermonde Matrix and Lagrange Polynomials}

We define the Vandermonde matrix of order $p$ ($p \in \NN^*$) of $x$ by
\eq{
	V_{p}^{x} = \left( (x_i)^j \right)_{i=1,\ldots,n}^{j=1,\ldots,p} =
	\begin{pmatrix}
		1 & x_1 & x_1^2 & \ldots & x_1^{p-1} \\
		1 & x_2 & x_2^2 & \ldots & x_2^{p-1} \\
		\vdots & \vdots & \vdots & \ddots & \vdots \\
		1 & x_{n} & x_{n}^2 & \ldots & x_{n}^{p-1} 
	\end{pmatrix}
	\in \RR^{n \times p}.
}

We define also what we call the derivative of order $l$ of the Vandermonde matrix of order $p$ of $x$ by
\eq{
	\pa{V_{p}^{x}}^{(l)} = \left( \pa{\frac{\d}{\d x_i} }^{l} \pa{(x_i)^{j-1}} \right)_{i=1,\ldots,n}^{j=1,\ldots,p}
	\in \RR^{n \times p}.
}

\begin{rem}
 If $p=n$, it is known that $V_{n}^{x}$ is invertible.
\end{rem}

The Vandermonde matrix is related to the Lagrange interpolation problem.
Indeed, if $b\in \RR^n$, the vector $a = (V_{n}^x)^{-1} b$ gives the coefficients of the unique polynomial $\pi_a\in \RR_{n-1}[X]$ satisfying
$\pi_a(x_j) = b_j$. There exists a formula to compute explicitly $\pi_a$ as follow using the Lagrange polynomials $(\ell_j^x)_{j=1}^{n}$
\eq{
	\pi_a(X) = \sum_i a_i X^i = \sum_{j} b_j \ell_{j}^x(X)
}
\eq{
	\qwhereq
	\ell_{j}^x(X) = \frac{\bar \ell_{j}^x(X) }{ \bar \ell_{j}^x(x_j) }, \quad
	\bar \ell_{j}^x(X) = \prod_{k \neq j} (X-x_k). 
}
In the following we write the expansion of the polynomial $\ell_j^x$ as 
\eq{
	\ell_j^x(X) = \sum_{i=1}^{n} \ell_{i,j}^x X^{i-1}
}
so that 
\eq{
	(V_{n}^x)^{-1} = ( \ell_{i,j}^x )_{i,j}.
}
Observe that the leading coefficient of $\ell_{j}^x$ is given by
\eq{
	\foralls j=1, \ldots, n, \quad
		\ell_{n,j}^x = \frac{1}{\bar \ell_{j}^x(x_j)}.
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Hermite Interpolation}

We define the matrix $H_{p}^x = \begin{pmatrix}
  V_p^{x}\\ \pa{V_p^x}'
\end{pmatrix} \in \RR^{(2n) \times p}$ where
\eq{
	\pa{V_p^x}' = 
	\begin{pmatrix}
		0 & 1 & 2 x_1 & \ldots & (p-1)x_1^{p-2} \\
		0 & 1 & 2 x_2 & \ldots & (p-1)x_2^{p-2} \\
		\vdots & \vdots & \vdots & \ddots & \vdots \\
		0 & 1 & 2x_{n} & \ldots & (p-1)x_{n}^{p-2} 
	\end{pmatrix}
	\in \RR^{n \times p}.
}

\begin{rem}
 If $p=2n$, then $H_{2n}^{x}$ is invertible.
\end{rem}

$H_{p}^x$ is the matrix associated to Hermite interpolation (i.e. interpolation of both the polynomial value and its derivative).
Indeed, one has that $a = (H_{2n}^x)^{-1} \begin{pmatrix}b\\c\end{pmatrix}$ are the coefficients of the polynomial $\pi_a(X)$ interpolating as follow
\eq{
	\pi_a(x_j) = b_j
	\qandq
	\pi_a'(x_j) = c_j.
}
There exists a formula to compute explicitly $\pi_a$ as follow using the Hermite polynomials $(\mu_j^x,\nu_j^x)_{j=1}^{n}$
\eq{
	\pi_a(X) = \sum_{i=1}^{2n} a_i X^{i-1} = \sum_{j=1}^{n} b_j \mu_j^x(X) + c_j \nu_j^x(X)
}
where
\begin{align*}
	\mu_{j}^x(X) &= \pa{ 1 - 2 (X-x_j) (\ell_{j}^x)'(x_j) } \ell_{j}^x(X)^2
		 = \sum_{i=1}^{2n} \mu_{i,j}^x X^{i-1}  \\
	\nu_{j}^x(X) &=  (X-x_j)  \ell_{j}^x(X)^2
		 = \sum_{i=1}^{2n} \nu_{i,j}^x X^{i-1}.
\end{align*}
with
\eq{
	(\ell_j^x)'(x_j) = \sum_{k \neq j} \frac{1}{x_j-x_k}.
}

This means that 
\eq{
	(H_{2n}^x)^{-1} = \left( 
			( \mu_{i,j}^x )_{1 \leq i \leq 2n}^{1 \leq j \leq n}, 
			( \nu_{i,j}^x )_{1 \leq i \leq 2n}^{1 \leq j \leq n}
		\right).
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Asymptotic of the Inverse Vandermonde and Hermite Matrices}

In this section we aim at describing the asymptotic behavior of the inverse of the matrices $V_{n}^{tx}$ and $H_{2n}^{tx}$ when $t>0$ is a parameter that tends to 
zero.

The next result, which is the key to our goal, describes an homogeneity property of the Lagrange and Hermite polynomials. It stems from the expression of those 
polynomials.

\begin{lem}\label{homogeneity}
One has for all $t>0$
\eq{
	\ell_{j}^{t x}(X) =  \ell_{j}^x(X/t)
\qarrq 
	\ell_{i,j}^{t x} = \ell_{i,j}^x t^{-(i-1)},
}
and
\eq{
	\choice{
		\mu_j^{tx}(X) = \mu_j^x(X/t), \\
		\nu_j^{tx}(X) = t\nu_j^x(X/t),
	}
	\qarrq
	\choice{
		\mu_{i,j}^{tx} = \mu_{i,j}^{x} t^{-(i-1)}, \\
		\nu_{i,j}^{tx} = \nu_{i,j}^{x} t^{-(i-2)}.
	}
}
\end{lem}

\begin{prop}\label{asympt_vanher}
 For all $t>0$, when $t$ tends to zero, one has the following asymptotic behavior of the inverse of the Vandermonde and Hermite matrices :

\eq{
	(V_{n}^{t x})^{-1} = 
	\frac{\Vv_x}{t^{n-1}} + O\pa{ \frac{1}{t^{n-2}} }
}
\eq{
	\qwhereq
	\Vv_x = 
	\begin{pmatrix}
		0 & 0 & \ldots & 0 \\
		\vdots & \vdots & \ddots & \vdots \\
		0 & 0 & \ldots & 0 \\
		\ell_{n,1}^x & 
		\ell_{n,2}^x & 
		\ldots &
		\ell_{n,n}^x & 
	\end{pmatrix},
}
and
\eq{
	(H_{2n}^{tx})^{-1} = 
	\frac{\Hh_x}{t^{2n-1}} + O\pa{ \frac{1}{t^{2n-2}} }
}
\eq{
	\qwhereq
	\Hh_x = 
	\begin{pmatrix}
		0 & \ldots & 0 & 0 & \ldots & 0 \\
		\vdots & \ddots & \vdots &  \vdots & \ddots & \vdots \\
		0 & \ldots & 0 & 0 & \ldots & 0 \\
		\mu_{2n,1}^x & 
		\ldots &
		\mu_{2n,n}^x & 
		0 &
		\ldots &
		0
	\end{pmatrix}.
}
\end{prop}

\begin{proof}
Thanks to Lemma \ref{homogeneity}, one has that for all $t>0$
\eq{
	(V_{n}^{tx})^{-1} = \left( 
				( \ell_{i,j}^x t^{-(i-1)} )_{1 \leq i \leq n}^{1 \leq j \leq n}
		\right)
}
and
\eq{
	(H_{2n}^{tx})^{-1} = \left( 
			( \mu_{i,j}^x t^{-(i-1)}   )_{1 \leq i \leq 2n}^{1 \leq j \leq n}, 
			( \nu_{i,j}^x t^{-(i-2)}   )_{1 \leq i \leq 2n}^{1 \leq j \leq n}
		\right)
}
hence the result.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Useful Matrix Results}

We now show some matrix results that we will use on the Gram matrix  $F_k^*F_k$ in order to have a precise description of its structure.


The next two propositions will be useful later on. Basically, we are interested in what we called a \emph{checkerboard} matrix and the structure of the set of those matrices.

\begin{defn}
 Let $n\in\NN^*$ and $A=(a_{i,j}) \in \RR^{n\times n}$. $A$ will be called a \emph{checkerboard} matrix if for all $(i,j)$ such that $i+j$ is odd, then $a_{i,j}=0$.
\end{defn}

Typically, for $n$ odd, such a matrix looks like :
\eq{
	\begin{pmatrix}
		a_{1,1} & 0 & a_{1,3} & 0 & \ldots & 0 & a_{1,n-2} & 0 & a_{1,n} \\
		0 & a_{2,2} & 0 & a_{2,4} & \ldots & a_{2,n-3} & 0 & a_{2,n-1} & 0 \\
		\vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots & \vdots \\
		0 & a_{n-1,2} & 0 & a_{n-1,4} & \ldots & a_{n-1,n-3} & 0 & a_{n-1,n} & 0 \\
		a_{n,1} & 0 & a_{n,3} & 0 & \ldots & 0 & a_{n,n-2} & 0 & a_{n,n}
	\end{pmatrix}
}

\begin{lem}\label{checkerboard_struct}
 The set of \emph{checkerboard} matrices of size $n \in \NN^*$ is an algebra over $\RR$.
\end{lem}
\begin{proof}
 The only difficulty is to show that the product of two checkerboard matrices is also a checkerboard matrix. Let $A=(a_{i,j})$ and $B=(b_{i,j})$ be two such matrices. Let $(i,j)$ such 
 that $i+j$ is odd. Then
 \eq{
	\sum_{k=1}^n a_{i,k}b_{k,j} =0
 }
 because if $i+k$ is even then $(i+j)-(i+k)=j-k$ is odd and $j-k+2k=j+k$ is odd, hence $b_{j,k}=0$. On the contrary, if $i+k$ is odd then $a_{i,k}=0$. So $AB$ is a checkerboard matrix. 
\end{proof}

Since the inverse of any matrix is a polynomial in that matrix, we immediately get :

\begin{cor}\label{checkerboard_inverse}
 The inverse of a \emph{checkerboard} matrix is also a \emph{checkerboard} matrix.
\end{cor}

\begin{lem}\label{damier_gramFk}
 For all $k\in \NN^*$, $F_k^* F_k$ is a checkerboard matrix.
\end{lem}

\begin{proof}
 Let $(i,j)$ such that $i+j$ is odd. The coefficient $(i,j)$ of $F_k^* F_k$ is equal to
 \eq{
	-\frac{1}{(i-1)!(j-1)!} \dotp{ \phi^{(i-1)} }{ \phi^{(j-1)} }
 }
 By successive integration by parts, one has that,
 \begin{align*}
	\dotp{ \phi^{(i-1)} }{ \phi^{(j-1)} } = (-1)^{j-1} \dotp{ \phi^{(i+j-2)} }{ \phi }, \\
	\dotp{ \phi^{(i-1)} }{ \phi^{(j-1)} } = (-1)^{i-1} \dotp{ \phi }{ \phi^{(i+j-2)} }.
 \end{align*}
 By the property of symmetry of the scalar product, if $\dotp{ \phi^{(i+j-2)} }{ \phi } \neq 0$, one gets that
 \eq{
	 (-1)^{i+j-2}=1,
 }
 which contradicts $i+j$ being an odd number. Thus $\dotp{ \phi^{(i+j-2)} }{ \phi } = 0$ and $\dotp{ \phi^{(i-1)} }{ \phi^{(j-1)} }=0$, hence the result.
\end{proof}


\begin{defn}
 Let $A \in \RR^{n\times n}$. We define the set of the anti-diagonals of $A$ by
 \eq{
	\Dd_A=\{d_1, \ldots, d_{2n-1}\},
 }
 where $d_i=(a_{k,j})_{k+j=i+1} \in \RR^{\max(i,i-2n+1)}$.
\end{defn}

\begin{rem}
 When $A$ is a checkerboard matrix then for all $i \in \NN^*$ such that $2i\leq n$, $d_{2i}=(0,\ldots,0)$.
\end{rem}

\begin{prop}
 Let $A=(a_{i,j})$ be a checkerboard matrix of size $2n+1$ such that $A$ is symmetric positive-definite and for all $i \in \{2j+1 ; \ 0\leq j \leq n \}$
 \eq{
	|a_{i,1}| >0 \qandq d_i=(-1)^{\frac{i-1}{2}} |a_{i,1}| (1,-1,\ldots,-1,1).
 }
 Let denote $B=(b_{i,j})=A^{-1}$.
 
 Then $b_{2n+1,2n+1}$ and $b_{1,2n+1}$ are positive.
\end{prop}

\begin{proof}
 The fact that $b_{2n+1,2n+1}$ is positive, is a direct consequence of the fact that $A^{-1}$ is symmetric positive-definite because so is $A$.
 
 Because of the inverse expression of a matrix thanks to the cofactor matrix, one has that $b_{1,2n+1}=\det(\hat{A}_{1,2n+1})/\det(A)$, where $\hat{A}_{1,2n+1}$ is the matrix 
 obtained from $A$ by removing the first row and the last column. Since $A$ is symmetric positive-definite, one has that $\det(A)>0$. So we need to show that $\det(\hat{A}_{1,2n+1})>0$. 
 But one can see that $\hat{A}_{1,2n+1}$ is a skew symmetric matrix of size $2n$, hence 
 \eq{
	\det(\hat{A}_{1,2n+1})=\mbox{pf}(\hat{A}_{1,2n+1})^2,
 }
 where $\mbox{pf}(\hat{A}_{1,2n+1})$ is the Pfaffian of the matrix $\hat{A}_{1,2n+1}$. Hence $\det(\hat{A}_{1,2n+1}) \geq 0$. For more details on the Pfaffian (definition and proof 
 of the result used here), see \cite{lang-algebra2002}. 
 
 Moreover one can see that $\hat{A}_{1,2n+1}$ is invertible. Indeed if we denote the colums of $A$ (resp. the columns $\hat{A}_{1,2n+1}$) as $C_1,\ldots,C_{2n+1}$ (resp. 
 $\hat{C}_1, \ldots,\hat{C}_{2n}$), one can see that for $0\leq i \leq n-1$, $\hat{C}_{2i+1}\in E_1$ and $\hat{C}_{2(i+1)}\in E_2$ where
 \begin{align*}
  E_1 &= \Span\{ e_{2j+1} ; \ 0 \leq j \leq n-1 \}, \\
  E_2 &= \Span\{ e_{2(j+1)} ; \ 0 \leq j \leq n-1 \},
 \end{align*}
 with $(e_i)_{1\leq i\leq 2n}$ is the canonical base of $\RR^{2n}$. Since $E_1$ and $E_2$ are in direct sum, if $\hat{A}_{1,2n+1}$ is not invertible it means that either 
 $(\hat{C}_{2i+1})_{0\leq i \leq n-1}$ or $(\hat{C}_{2(i+1)})_{0\leq i \leq n-1}$ is linearly dependent. But it can not be $(\hat{C}_{2(i+1)})_{0\leq i \leq n-1}$ because it would 
 imply that $(C_{2(i+1)})_{0\leq i \leq n-1}$ is also linearly dependent, because
 \eq{
	C_{2(i+1)}=\begin{pmatrix}
	                0 \\
	                \hat{C}_{2(i+1)}
	             \end{pmatrix},
 }
 which would contradict the invertibility of $A$.
 
 So it means that $(\hat{C}_{2i+1})_{0\leq i \leq n-1}$ must be linearly dependent. However from the structure of the matrix $A$, one can see that for all $0\leq i \leq n-1$
 \eq{
  \hat{C}_{2i+1}=
  \begin{pmatrix}
   0 \\
   (-1)^{i+1} a_{2i+1,1} \\
   0 \\
   -(-1)^{i+1} a_{2i+3,1} \\
   \vdots \\
   0 \\
   (-1)^{i+1} a_{2(i+n)-1,1} \\
   0 \\
   -(-1)^{i+1} a_{2(i+n)+1,1} 
  \end{pmatrix}
  \qandq
  \hat{C}_{2(i+1)}=
  \begin{pmatrix}
   (-1)^{i+1} a_{2i+1,1} \\
   0 \\
   -(-1)^{i+1} a_{2i+3,1} \\
   0 \\
   \vdots \\
   (-1)^{i+1} a_{2(i+n)-1,1} \\
   0 \\
   -(-1)^{i+1} a_{2(i+n)+1,1} \\
   0
  \end{pmatrix}.
 }
 Thus, a linear combination between the elements of $(\hat{C}_{2i+1})_{0\leq i \leq n-1}$ gives the same linear combination between the elements of 
 $(\hat{C}_{2(i+1)})_{0\leq i \leq n-1}$, which contradicts for the same reason as before the invertibility of $A$.
 
 Hence $\hat{A}_{1,2n+1}$ is invertible and $b_{1,2n+1}>0$.
\end{proof}





==> sections/aux/sec-proof-thm.tex <==
% !TEX root = ../article-asymptotic.tex
\section{Proof of Theorem~\ref{thm-main}}
\label{main}


The proof of this theorem is divided in two parts.
In the first part, we use the implicit function theorem to construct an potential solution. The main difficulty in this part is that the first order condition of BLASSO restricted to exact support recovery leads to a degenerate functional, that needs to be de-singularized to be able to apply the implicit function theorem. 
In the second part, we prove that this candidate solution is indeed a solution, which requires some technical asymptotic analysis of the various quantities involved. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Construction of a Candidate Solution} 

Since a discrete measure $m=m_{\ta,\tx}$ is a solution of $(P_\lambda(y+w))$ if and only if there exists $\eta \in \Cc(\TT)$ such that
\eq{
	\Phi^*(\Phi m - \Phi_{tx} a - w) + \lambda \eta=0,
}
with $\normi{\eta} \leq 1$ and $\eta(\tx)=\sign(\ta)$ (ie $\eta \in \partial \normTV{m_{\ta,\tx}}$), it is natural to look for a solution $m_{\ta,\tx}$ with $n$ spikes among those which
verify the following two equations 
\begin{align*}
 \Phi_{\tx}^*(\Phi_{\tx} \ta - \Phi_{tx} a - w) + \lambda \sign(a)&=0 \\
 (\Phi_{\tx}^*)'(\Phi_{\tx} \ta - \Phi_{tx} a - w)&=0
\end{align*}
which means that $\eta_\lambda(\tx)=\sign(a)$ and $\eta_\lambda'(\tx)=0$ where $\eta_\lambda=\frac{1}{\lambda} \Phi^*(\Phi_{tx} a + w - \Phi_{\tx}\ta)$.

The above two equations can be rewritten as
\begin{align}\label{eqn_implicit}
	E(\tu,\theta)&=0,
\end{align}
where $\tu=(\ta,\tx)$, $\theta=(\lambda,w,t)$ and $E(\tu,\theta)=\Ga_{\tx}(\Phi_{\tx} \ta - \Phi_{tx} a - w) + \lambda \alpha_n$. Moreover the set of solution of equation 
\eqref{eqn_implicit} is not empty because $E(a,0,0,0,0)=0$.

The idea is to build a candidate solution by applying the implicit function theorem to $E$ at the point $((a,0),0)$ which would in turn defines a parametrization of 
$\tu=(\ta,\tx)$ with respect to $\theta$ around $\theta=(0,0,0)$. Then one has to check that the obtained measure $m_{\ta,\tx}$ is indeed a solution of $P_\lambda(y+w)$ by verifying 
that $\normi{\eta_\lambda}\leq 1$ (because we already know that the other condition on $\eta_\lambda$ is true by construction of $\tu$). But that is the second and last part of the 
proof. Now we focus on the use of the implicit function theorem.

\bigskip

First we introduce the following change of variables
\eq{
	(\ta,\tx)=(a+t^\al \de,t x + t^\al \mu)
	\qandq
	(\la, w, t) = (t^{\be-1} \ga, t^\be \epsilon,t).
}
for some $\al>1$ and $\be \geq \al$ that we choose later on. This is natural to consider because we expect the solution to the BLASSO to be close to the input measure when the noise 
and the regularization parameter are small enough with respect to a certain exponent of $t$. We denote $(v,\xi)$ the new variables and 
$\hat E(v,\xi)=E((a+t^\al \de,t x + t^\al \mu),(t^\be \ga, t^\be \epsilon,t))$.

One cannot apply directly the implicit function theorem to $\hat E$ at $(v,\xi)=(0,0)$ because $\frac{\partial \hat E}{\partial v}(0,0)=0$. The idea is to apply the implicit function 
theorem to a function which admits the same solution as equation \eqref{eqn_implicit} but with an invertible partial derivative with respect to $v$ at $(0,0)$. A solution is to 
consider
\eq{
	F(v,\xi)=\frac{1}{t^\alpha}D_{a}^{-1}(\Ga_{tx}^*\Ga_{tx})^{-1} \hat E(v,\xi).
}
Because $\frac{1}{t^\alpha}D_{a}^{-1}(\Ga_{tx}^*\Ga_{tx})^{-1}$ is invertible, the solutions to $F(v,\xi)=0$ are the same as those of $\hat E(v,\xi)=0$. Moreover one has the 
following result :

\begin{lem}\label{tfi}
 $F$ is a $\Cc^1$ function around $(0,0)$ and $\frac{\partial F}{\partial v}(0,0)$ is invertible.
\end{lem}

\begin{proof}
 The proof of this lemma is not complete, everything is not yet justified. But it seems that our change of variable and the function $F$ considered represents the right choice. The 
 computations give us with $\al>4n-2$, $\beta=\al+2n-1$ and thanks to Theorem \ref{behavior_pinvGa}, \ref{behavior_biais}
 \begin{align*}
  \pd{F}{v}(v,\xi) &= \Id + O( t^{\al - 4n + 2} ) = \Id+O(t) \\
  \pd{F}{t}(v,\xi) &= s_{x} + O(t) \\
	%
	\pd{F}{\epsilon}(v,\xi) &= -t^{\be-\al} D_{a}^{-1}\Ga_{tx}^+ + O(t) 
		= -D_{a}^{-1}\Hh_x F_{2n}^+ + O(t) \\
	%
	\pd{F}{\ga}(v,\xi) &= t^{\be-1-\alpha}D_{a}^{-1} (\Ga_{tx}^* \Ga_{tx})^{-1} \al_n = D_{a}^{-1} r_{x} + O(t).
 \end{align*}

\end{proof}

So we can apply the implicit function theorem to $F$ at $(0,0)$ and thanks to the derivative of $F$ obtained from the lemma, one gets
\eq{
	\begin{pmatrix}
		\ta \\
		\tx 
	\end{pmatrix}
	= 
	\begin{pmatrix}
		a \\
		t x
	\end{pmatrix}
	-
	\frac{D_{a}^{-1}}{t^{2n-1}}
	\pa{
		\Hh_x F_{2n}^+ w
	-	t\la r_{x} 
	}
	+ 
	s_{x} t^{\al+1}
	+ o\pa{t^{\al+1}, \frac{\norm{w},\la}{t^{2n-1}} 
		}.
 }

Now, we need to prove that the constructed candidate solution is in fact a solution. It is the second step of the theorem proof.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Checking the BLASSO First Order Conditions} 

We provide only the main idea of the proof, there is still work to do.

In order to prove that $m_{\ta,\tx}$ is indeed a solution of $(P_\lambda(y+w))$, one must verify that 
$\normi{\eta_\lambda}\leq 1$. We use the Vanishing pre-certificate associated to the input measure $m_{a,tx}$ (see \cite{duval-exact2013}) which is defined by
\eq{
	\eta_{V,t}=\Phi^*\Ga_{tx}^{+,*}\al_n.
}
First we need to check that 
\eq{
	\foralls k, \quad \norm{ \eta_\la^{(k)} - \eta_{V,t}^{(k)} } = O\pa{ \normd{w}/\la,\la }
}
Hence $\eta_\la''$ is close to $\eta_{V,t}''=(\Phi^*)'' \Ga_{tx}\al_n$ provided that $\normd{w}/\la$ and $\la$ are small enough. But thanks to Theorem \ref{exp_etaV}, we know that 
$\eta_{V,t}$ is concave around the points $tx_i$, hence so is $\eta_\la$.

Then we can show the desired result.

==> sections/aux/sec-support-recovery.tex <==
% !TEX root = ../article-asymptotic.tex
\section{Exact Support Recovery}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Vanishing Derivative Certificates}


Following~\cite{duval-exact2013}, we introduce below the so called ``vanishing pre-certificate'' $\eta_{V,t}$, which is a function defined on $\TT$ that interpolates the spikes positions and signs (here $+1$). Note that $\eta_{V,t}$ can be computed in closed form by solving a linear system~\cite{duval-exact2013}.

\begin{defn}[Vanishing pre-certificate]
Let $\eta_{V,t}=\Phi^* p_{V,t}$ where
\begin{align*}
  	p_{V,t}=\underset{p\in L^2(\TT)}{\argmin} \left\{\normd{p}; \ (\Phi^*p)(t x_{i})=1 \mbox{ and } (\Phi^*p)'(t x_{i})=0~\forall i\right\}.
\end{align*}
\end{defn}

If $\normi{\eta_{V,t}} \leq 1$, it can be shown that $m_{a,tx}$ is recovered by the BLASSO when $(\la,w)=(0,0)$. 
We say that $\eta_{V,t}$ is \textit{non degenerate} if furthermore $|\eta_{V,t}|<1$ outside the position $tx_i$ and $\eta_{V,t}''(tx_i) \neq 0$. It is shown in~\cite{duval-exact2013} that $\eta_{V,t}$ being non-degenerated implies that solving~\eqref{blasso} for a well chosen $\la$ gives a solution with the correct number $n$ of spikes, i.e. one obtain exact support recovery.


%As a consequence, $\eta_{V,t}$ is a certificate of the Basis Pursuit $(\Pp_0(y))$ for the initial measure $m_{a,tx}$ if and %only if $\normi{\eta_{V,t}}\leq 1$. Moreover if $\eta_{V,t}$ is non-degenerated i.e.
%\begin{align*}
%	\forall u\in \TT-\{tx_1,\ldots,tx_n\}, \ |\eta_{V,t}(u)|<1,
%\end{align*}
% then it controls the recovery property of the support of the solution of the BLASSO in a low-noise regime (see \cite{duval-exact2013}). As we want to determine the asymptotic behavior of the recovery of $m_{a,tx}$ when solving $(\Pp_\lambda(y+w))$, we have to look at $\underset{t\rightarrow 0}{\lim} \ \eta_{V,t}$.

Figure~\ref{certif-convergence}, top row, shows graphically that $\eta_{V,t}$ converges with $t \rightarrow 0$ toward a fixed function $\eta_W$ that does not depend on $x$ and $t$. This function is defined in the following proposition, which ensures that the non-degeneracy of $\eta_{V,t}$ can thus be checked independently of $x$ and $t$ provided that $t$ is small. 

\begin{prop}
	One has the uniform convergence $\eta_{V,t} \rightarrow \eta_W = \Phi^* p_{W}$ as $t \rightarrow 0$, where
	\begin{align*}
  		p_W \!=\! \underset{p\in L^2(\TT)}{\argmin} \left\{\normd{p}; (\Phi^*p)(0)=1, (\Phi^*p)^{(i)}(0)=0~\forall i\leq 2n-1\right\}.
	\end{align*}	
	Furthermore, if $|\eta_W|<1$ outside $0$ and $\eta_W^{(2n)}(0) \neq 0$ (we then say that $\eta_W$ is $(2n)$-non-degenerated), then $\eta_{V,t}$ is non degenerated for small $t$. 
\end{prop}

Figure~\ref{certif-convergence}, bottom row, shows $\eta_W$ for several values of $n$. Note how it becomes flatter at $0$ as $n$ increases. This implies that $\eta_{V,t}$ for small $t$ gets closer to degeneracy at $N$ increases. This is reflected in our main contribution (Theorem~\ref{thm-main} bellow) where signal-to-noise ratio is required to scale like $1/t^{2N-1}$.

% In the following Proposition, we show that the non-degeneracy of $\eta_{V,t}$ does not depend on $t$ (i.e. the minimum separation) for positive measures but only on the filter $\phi$. 

% \begin{proposition}
% If for all $u\in \TT-\{0\}$, one has $|\eta_W(u)|<1$ then there exists $t_0>0$ such that for all $t \in ]0,t_0[$, $\eta_{V,t}$ is non-degenerate.
% \end{proposition}


\begin{figure*}
	\centering    
	\begin{tabular}{@{\hspace{1mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{1mm}}}
      \includegraphics[width=0.32\linewidth]{certif-convergence/certif-convergence-3} &
      \includegraphics[width=0.32\linewidth]{certif-convergence/certif-convergence-5} &
      \includegraphics[width=0.32\linewidth]{certif-convergence/certif-convergence-7} \\
      $t=0.4$ & $t=0.2$ & $t=0.01$ \\
      \includegraphics[width=0.32\linewidth]{asymptotic-certif/asymptotic-certif-1}&
      \includegraphics[width=0.32\linewidth]{asymptotic-certif/asymptotic-certif-2}&
      \includegraphics[width=0.32\linewidth]{asymptotic-certif/asymptotic-certif-3}\\
      $n=1$ ($\eta_{V,t}=\eta_W$) & $n=2$ & $n=3$
   	\end{tabular}
\caption{\label{certif-convergence} 
	\textit{Top row:} $\eta_{V,t}$ for several values of $t$, showing the convergence toward $\eta_W$. 
	The filter $\phi$ is an ideal low-pass filter with a frequency cutoff $f_c=10$.
	\textit{Bottom row:}  $\eta_W$ for several value of $n$. 
}
\end{figure*}
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Main Contribution}

Our main contribution is the following Theorem. 

\todo{fuse the following}



\begin{thm}
If $\eta_W$ is $(2n)$-non-degenerated, then for $(\frac{\norm{w}}{\lambda},\frac{\norm{w}}{t^{2n-1}},\frac{\lambda}{t^{2n-2}},t)= O(1)$, the solution $m_{a^\star,x^\star}$ of~\eqref{blasso} for small enough $t$ is unique and composed of $n$ spikes. Moreover one has the following first order expansion of the amplitudes and positions of the recovered measure 
\begin{equation}
	(a^\star,x^\star) = 
 (a,tx) + A_x \frac{w}{t^{2n-1}} + B_x \frac{\lambda}{t^{2n-2}} + R(w,\lambda,t),
\end{equation}
where $A_x : \Ldeux(\TT) \rightarrow \RR^{2n}$ and $B_x \in \RR^{2n}$ are constants\footnote{With explicit expressions, not provided here due to lack of space.}, and $R(w,\lambda,t)$ is negligible with respect to the first order terms.
\end{thm} 



\begin{thm}\label{thm-main}
 If $\Cc_{2n}$ holds then there exists $\lambda_0>0$, $t_0>0$, $c_\lambda>0$ and $c_t>0$ such that for all $(\lambda,w,t) \in \RR_+ \times \Ldeux(\TT) \times \RR_+$ verifying 
 \begin{align*}
  & 0 < \lambda < \lambda_0 \\
  & 0 < t < t_0 \\
  & \normd{w}\leq c_w \lambda \\
  & \normd{w}\leq c_t t^{2n-1}
 \end{align*}
 the problem $(\Pp_\lambda(y+w))$, where $y=\Phi m_{a,tx}=\Phi_{tx} a$, admits a unique solution composed of exactly $n$ spikes given by $m_{\ta,\tx}=\sum_{i=1}^n \ta_i \de_{\tx_i}$. 
 Moreover $(\ta,\tx)$ are given by the following expansion for all $\al > 4n-2$
 \eq{
	\begin{pmatrix}
		\ta \\
		\tx 
	\end{pmatrix}
	= 
	\begin{pmatrix}
		a \\
		t x
	\end{pmatrix}
	-
	\frac{D_{a}^{-1}}{t^{2n-1}}
	\pa{
		\Hh_x F_{2n}^+ w
	-	t\la r_{x} 
	}
	+ 
	s_{x} t^{\al+1}
	+ o\pa{t^{\al+1}, \frac{\norm{w},\la}{t^{2n-1}} 
		}.
 }
 where $D_a=\text{diag}(Id,\text{diag}(a))$, $r_x$ and $s_x$ are constants vectors that we define in the following.
\end{thm}

The proof of this Theorem can be found in Section~\ref{}.

